Task-Graph Scheduling Extensions for Efficient Synchronization and Communication

Task graphs have been studied for decades as a foundation for scheduling irregular parallel applications and incorporated in programming models such as OpenMP. While many high-performance parallel libraries are based on task graphs, they also have additional scheduling requirements, such as synchronization from inner levels of data parallelism and internal blocking communications. In this paper, we extend task-graph scheduling to support efficient synchronization and communication within tasks. Our scheduler avoids deadlock and oversubscription of worker threads, and refines victim selection to increase the overlap of sibling tasks. To the best of our knowledge, our approach is the first to combine gang-scheduling and work-stealing in a single runtime. Our approach has been evaluated on the SLATE highperformance linear algebra library. Relative to the LLVM OMP runtime, our runtime demonstrates performance improvements of up to 13.82%, 15.2%, and 36.94% for LU, QR, and Cholesky, respectively, evaluated across different configurations.

==> Makefile <==
LATEX=latexmk
LATEXMKOPTS = -bibtex -pdf -halt-on-error -interaction=nonstopmode

PAPER=paper
SUB=submission/paper
DIFF=diff

TEXFILES = *.tex

all: paper 

paper: $(TEXFILES) FORCE_MAKE
	$(LATEX) $(LATEXMKOPTS) $(PAPER)
#	cp paper.pdf ../
#	pdflatex paper.tex
#	bibtex paper
#	pdflatex paper.tex
#	pdflatex paper.tex
#	pdflatex paper.tex


diff: $(TEXFILES) clean FORCE_MAKE
	latexdiff --config='PICTUREENV=(?:picture|DIFnomarkup|lstlisting|tabular)[\w\d*@]*' --flatten --type=BOLD $(SUB).tex $(PAPER).tex > $(DIFF).tex
	sed '/DeclareOldFontCommand/c \\\DeclareOldFontCommand{\\bf}{\\color{blue}\\normalfont}{\\mathbf}' $(DIFF).tex > $(DIFF)_refined.tex
	$(LATEX) $(LATEXMKOPTS) $(DIFF)_refined.tex

clean:
	$(LATEX) -C
	rm -f *.bbl
	rm -f *.cb
	rm -f *.cb2
	rm -f $(DIFF).tex

.PHONY: clean FORCE_MAKE


==> ack.tex <==
This research was supported by the Exascale Computing Project
(17-SC-20-SC), a collaborative effort of the U.S. Department of Energy
Office of Science and the National Nuclear Security Administration,
       and by the U.S. Department of Energy, Office of Science, under
       Contract DE-AC02-06CH11357. We gratefully acknowledge the computing
       resources provided and operated by the Joint Laboratory for System
       Evaluation (JLSE) at Argonne National Laboratory.

